When Rigidity Hurts: Soft Consistency Regularization for Probabilistic Hierarchical Time Series Forecasting

Probabilistic hierarchical time-series forecasting is an important variant of time-series forecasting, where the goal is to model and forecast multivariate time-series that have underlying hierarchical relations. Most methods focus on point predictions and do not provide well-calibrated probabilistic forecasts distributions. Recent state-of-art probabilistic forecasting methods also impose hierarchical relations on point predictions and samples of distribution which does not account for coherency of forecast distributions. Previous works also silently assume that datasets are always consistent with given hierarchical relations and do not adapt to real-world datasets that show deviation from this assumption. We close both these gap and propose PROFHiT, which is a fully probabilistic hierarchical forecasting model that jointly models forecast distribution of entire hierarchy. PROFHiT uses a flexible probabilistic Bayesian approach and introduces a novel Distributional Coherency regularization to learn from hierarchical relations for entire forecast distribution that enables robust and calibrated forecasts as well as adapt to datasets of varying hierarchical consistency. On evaluating PROFHiT over wide range of datasets, we observed 41-88% better performance in accuracy and significantly better calibration. Due to modeling the coherency over full distribution, we observed that PROFHiT can robustly provide reliable forecasts even if up to 10% of input time-series data is missing where other methods' performance severely degrade by over 70%.

==> Text/abstract.tex <==
\begin{abstract}

  Probabilistic hierarchical time-series forecasting is an important variant
  of time-series forecasting, where the goal is to model and forecast
  multivariate time-series that have underlying hierarchical relations. Most
  methods focus on point predictions and do not provide well-calibrated
  probabilistic forecasts distributions. Recent state-of-art probabilistic
  forecasting methods also impose hierarchical relations on point predictions
  and samples of distribution which does not account for coherency of forecast
  distributions.
  Previous works also silently assume that datasets are always consistent with given hierarchical relations
  and do not adapt to real-world datasets that show deviation from this assumption.
  %\zc{Change this sentence to emphasize previous methods do
  %  not model the coherency very well, align with your introduction
  %  structure. }  
  We close both these gap and propose \model, which is a fully
  probabilistic hierarchical forecasting model that jointly models forecast
  distribution of entire hierarchy. \model uses a flexible probabilistic Bayesian approach
  and introduces a novel Distributional
  Coherency regularization to learn from hierarchical relations for entire
  forecast distribution that enables robust and calibrated forecasts as well as
  adapt to datasets of varying hierarchical consistency.
  %\zc{The selling over method is still too simple you
  %  need to sell According to our key technical innovations for For addressing
  %    the two gaps: coherency and robustness. . }
  On evaluating \model over wide range of datasets, we
  observed 41-88\% better performance in accuracy and significantly better calibration. Due to
  modeling the coherency over full distribution, we observed that \model can
  robustly provide reliable forecasts even if up to 10\% of input time-series
  data is missing where other methods' performance severely degrade by over
  70\%.

\end{abstract}

==> Text/checklist.tex <==
\section*{Checklist}


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{Mentioned in the README of code}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


==> Text/dump.tex <==
\section{Derivation of distributional coherency loss}
We derive the equation \ref{eqn:jsd} that defines the distributional coherency loss.
We use the following result for KL-Divergence of two Gaussian Distributions.
\begin{lemma}
    Given two univariate Normal distributions $P_1 = \mathcal{N}_1(\mu_1, \sigma_1)$ and $P_2 = \mathcal{N}_2(\mu_2, \sigma_2)$, the KL-Divergence is
    \begin{equation}
        \begin{split}
            D_{KL}(P_1||P_2) = \frac{1}{2} \left[ 2\log \frac{\sigma_2}{\sigma_1} + \frac{\sigma_1^2 + (\mu_1 -\mu_2)^2}{\sigma_2^2} - 1 \right]
        \end{split}
    \end{equation}
    \label{lemma:kl}
\end{lemma}

Jenson Shannon Divergence between two distributions $P_1$ and $P_2$ is defined as
\begin{equation}
    JSD(P_1, P_2) = \frac{1}{2} \left( D_{KL}(P_1||P_2) + D_{KL}(P_2||P_1) \right).
\end{equation}

Using Lemma \ref{lemma:kl} we have
\begin{corollary}
    Given two univariate Normal distributions $P_1 = \mathcal{N}_1(\mu_1, \sigma_1)$ and $P_2 = \mathcal{N}_2(\mu_2, \sigma_2)$, the JSD is
    \begin{equation}
        JSD(P_1,P_2) = \frac{1}{2} \left[\frac{\sigma_1^2 + (\mu_1 -\mu_2)^2}{2\sigma_2^2} + \frac{\sigma_2^2 + (\mu_1 -\mu_2)^2}{2\sigma_1^2} - 1\right]
    \end{equation}
    \label{corr:jsd}
\end{corollary}

Consider each term $JSD(P(y_i^{t+\tau}|\basemu_i, \basesigma_i), P(\sum_{j\in \mathbf{C}_i}\phi_{ij} y_j^{t+\tau}| \{|\basemu_j, \basesigma_j\}_{j\in \mathbf{C}_i} )) + 1$ of $\mathcal{L}_2$. Note that \[P(y_i^{t+\tau}|\basemu_i, \basesigma_i) = \mathcal{N}(\mu_i,\sigma_i)\] and $P(\sum_{j\in \mathbf{C}_i}\phi_{ij} y_j^{t+\tau}| \{|\basemu_j, \basesigma_j\}_{j\in \mathbf{C}_i} ))$ is sum of random variables $\{\phi_{ij}\mathcal{N}(\mu_j, \sigma_j)\}_{j\in C_i}$. Therefore


\[P(\sum_{j\in \mathbf{C}_i}\phi_{ij} y_j^{t+\tau}| \{|\basemu_j, \basesigma_j\}_{j\in \mathbf{C}_i} )) = \mathcal{N}(\sum_{j\in C_i} \phi_{ij} \mu_j, \sqrt{\sum_{j\in C_i} \phi_{ij} \sigma_j^2})\]

Then using Corollary \ref{corr:jsd}, we get the desired expression of Equation \ref{eqn:jsd}, rewritten below:
\begin{equation}
    \begin{split}
        \mathcal{L}_2 &= 2\left[\sum_{i=1}^N JSD(P(y_i^{t+\tau}|\basemu_i, \basesigma_i), P(\sum_{j\in \mathbf{C}_i}\phi_{ij} y_j^{t+\tau}| \{|\basemu_j, \basesigma_j\}_{j\in \mathbf{C}_i} )) + 1\right]\\
        &= \sum_{i=1}^N \left[\frac{\sigma_i^2 + \left( \mu_i - \sum_{j\in C_i} \phi_{ij}\mu_j \right)^2}{2\sum_{j\in C_i}\phi_{ij} \sigma_j^2} + \frac{\sum_{j\in C_i}\phi_{ij} \sigma_j^2 + \left( \mu_i - \sum_{j\in C_i} \phi_{ij}\mu_j \right)^2}{2\sigma_i^2} \right]
    \end{split}
\end{equation}



We use the following well-known result for KL-Divergence of two Gaussian Distributions.
\begin{lemma}
    Given two univariate Normal distributions $P_1 = \mathcal{N}_1(\mu_1, \sigma_1)$ and $P_2 = \mathcal{N}_2(\mu_2, \sigma_2)$, the KL-Divergence is
    \begin{equation}
        \begin{split}
            D_{KL}(P_1||P_2) = \frac{1}{2} \left[ 2\log \frac{\sigma_2}{\sigma_1} + \frac{\sigma_1^2 + (\mu_1 -\mu_2)^2}{\sigma_2^2} - 1 \right]
        \end{split}
    \end{equation}
    \label{lemma:kl}
\end{lemma}

Note that, $JSD$ between two distributions $P_1$ and $P_2$ is defined as
\begin{equation}
    JSD(P_1, P_2) = \frac{1}{2} \left( D_{KL}(P_1||P_2) + D_{KL}(P_2||P_1) \right).
\end{equation}

Using Lemma \ref{lemma:kl} we have the following result for $JSD$.
\begin{corollary}
    Given two univariate Normal distributions $P_1 = \mathcal{N}_1(\mu_1, \sigma_1)$ and $P_2 = \mathcal{N}_2(\mu_2, \sigma_2)$, the JSD is
    \begin{equation}
        JSD(P_1,P_2) = \frac{1}{2} \left[\frac{\sigma_1^2 + (\mu_1 -\mu_2)^2}{2\sigma_2^2} + \frac{\sigma_2^2 + (\mu_1 -\mu_2)^2}{2\sigma_1^2} - 1\right]
    \end{equation}
    \label{corr:jsd}
\end{corollary}

\iffalse
    {\footnotesize
    \begin{equation}
        \begin{split}
            P(\{y_i^{t+\tau}\}_{i=1}^N| \mathcal{D}_t) &=
            \int \underbrace{\left( \prod_{i=1}^{N}  P(\mathbf{u_i}|\mathbf{y_i^{(t':t)}})  \prod_{i=1}^{N}  P(\mathbf{u'_i}|\mathbf{y_i^{(1:t)}}) \right)}_{\text{\camul (Raw Forecasts)}}
            \underbrace{P(\mathbf{z}|\{\mathbf{u'_i}\}) \left(\prod_{i=1}^{N} P(\mathbf{z_i}|\{\mathbf{u'_i}, \mathbf{u_i}\}_{i=1}^N) P(\basemu_i, \basesigma_i|\mathbf{z}_i, \mathbf{z}, \mathbf{u}_i) \right)}_{\text{\camul (Raw forecasts)}} \\
            &\underbrace{\prod_{i=1}^N P(\mu_i, \sigma_i| \{\basemu_j, \basesigma_j\}_{j=1}^N) P(y_i^{t+\tau}|\mu_i, \sigma_i)}_{\text{Refinement Module}} d\{\mathbf{u_i}\}_{i=1}^N d\{\mathbf{z_i}\}_{i=1}^N.
        \end{split}
        \label{eqn:process1}
    \end{equation}
    }
\fi

==> Text/intro_dump.tex <==
\section{Introduction}

Time-series forecasting is an important problem that impacts decision-making in a wide range of applications.
In many real-world situations, the time-series have inherent hierarchical
relations and structures.
Examples  include forecasting time-series of
employment  \citep{taieb2017coherent} measured at different
geographical scales; epidemic forecasting \citep{reich2019collaborative} at county, state and country, etc.
% The time-series values follow these hierarchical relations with varying degree of \textbf{consistency}.  \zc{why bold font?} 
% Data at lower levels of hierarchy
% usually contain complex patterns, and leveraging the hierarchy to
% provide coherent forecasts allows for better performance than independently
% modeling individual time-series. 
%Hierarchical Time-series Forecasting (\htsf)
%aims to effectively model multiple time-series whose values at any given time-step is consistent with given
%hierarchical relations. 
Given time-series dataset with underlying hierarchical relations, the goal of Hierarchical Time-series Forecasting (\htsf) is to generate accurate forecast for all time-series leveraging the hierarchical relations between time-series  \citep{hyndman2011optimal}.
%Generating \htsf forecasts that satisfy these
%hierarchical relations is said to be \textit{coherent}
%\citep{rangapuram2018deep} and it is a desirable goal in many applications.
%sales demand data at multiple spatial scales 

% The hierarchical relation in most cases is a simple or weighted summation. For instance, the retail sales in a given state is the sum of retail demand over all counties of the state. Similarly, number of hospitalizations or cases for a disease in a country is sum of cases in each of its provinces.

%\zc{better to choose two or three examples and
%expand them, decribe what htf means in such examples}  


Most previous methods are not designed to provide \textit{well-calibrated} forecasts for \textit{both} so-called \textit{"strong"} and \textit{"weakly" consistent} datasets.
Previous \htsf methods assume that the dataset is strongly consistent:
the time-series values of datasets strictly satisfy
the underlying hierarchical constraints. The models impose \textit{rigid}
\textit{coherency} on generated forecasts i.e., forecasts strictly satisfy the hierarchical relations of dataset.
These methods can model  datasets generated
\citep{taieb2017coherent} by first collecting data for time-series of the leaf
level nodes  and deriving time-series for higher-level nodes.
%For example, the well-studied \wiki dataset
%\citep{taieb2017coherent} contains visit counts for 150 groups of articles and
%these values are further aggregated by topic similarity to form a 4-level
%hierarchy.
We call such data as \textit{strongly consistent}.
For example, classical
\htsf~ methods~\citep{hyndman2018forecasting}
use a bottom-up or top-down approach where all time-series at a
single level of hierarchy are modeled
independently and the values of other levels are derived using
the aggregation function governing the hierarchy.
\zc{try to simplify the first half this paragraph, just say most existing methods imposes rigid coherency, namely XX. They use top-down or bottom-up XXX. However, in many applications, the time series data are weakly coherent. PS, try to use just either coherency or consistency.}
%Other methods revise forecasts full hierarchy simultaneously to be fully coherent.
In contrast, many real-world
datasets are \textit{weakly consistent}, i.e., they do not follow the strict
constraints of the hierarchy\footnote{Note that we describe \emph{consistency} over a dataset and \emph{coherency} over model forecasts.}.
Such data have an underlying data generation
process that may follow a hierarchical set of constraints but may contain some deviations.
These deviations can be caused by factors such as
measurement or reporting error, asynchrony in data aggregation and revision
pipeline, etc, as frequently observed in epidemic forecasting \citep{adhikariKDD2019}. %and are usually more pronounced at leaf nodes of the hierarchy.
%For example, in the case of epidemic %forecasting~\citep{adhikariKDD2019}, data
%at the county and state levels have higher noise and discrepancies %compared to
%data at the national level. 
Most state-of-the-art \htsf methods are
designed for strongly consistent datasets and impose rigid coherency constraints --- they thus may not adapt to such
deviations and can \textit{provide poor forecasts for weakly consistent datasets}
\zc{don't say dataset, say relations or applications} .


%\aditya{can we make the paragraph more succint? so While these methods are .., they impose coherenct only on point predictions (e.g. by linear ...) or fiixed ... (e.g.)} 
\input{Text/first_fig}
Moreover, previous methods do not focus on providing \textit{calibrated forecasts} with precise uncertainty measures.
Traditional methods focus on point predictions only.
Recent methods like \mint \citep{wickramasuriya2019optimal}, \erm \citep{ben2019regularized} and \pembu \citep{taieb2017coherent}
refine raw independent forecast distribution as a post-processing step. This does not enable the models generating the raw forecasts to leverage underlying hierarchical relations across time-series.
End-to-end learning neural methods  directly leverage hierarchical relations as part of the model architecture or learning algorithm like \hiere \citep{rangapuram2021end} and \sharq \citep{han2021simultaneously}. They do this and usually outperform post-processing methods by imposing hierarchical constraints on the mean or fixed quantiles of the forecast distributions.
%While recent works on probabilistic
%\htsf propose deep-learning approaches for modeling all time-series of the
%hierarchy simultaneously, they impose coherency on point predictions only by
%sampling from distributions \citep{rangapuram2021end} or quantiles of
%distributions \citep{han2021simultaneously}. %while other non-parametric density estimation methods leverage specific domain knowledge \citep{taieb2021hierarchical}. 
However, these methods do not enforce hierarchical coherency on the full distributions.
Therefore, the \textit{forecasts may not be well-calibrated} \citep{kuleshov2018accurate} i.e., they produce unreliable prediction intervals that may not match observed probabilities from ground truth \citep{fisch2022calibrated}.
%We also observe lack of coherency and calibration on full distributions also effects the \textit{robustness} of the models i.e., the ability to perform well in presence noise and missing data.
%\zc{what's the key message you want to convey is this paragraph?} 

\input{Text/table_first}

In this work, we fill this gap of learning well-calibrated and accurate forecasts for both strong and weakly consistent datasets leveraging underlying hierarchical relations.
We propose \model (\underline{P}robabilistic \underline{Ro}bust \underline{F}orecasting for \underline{Hi}erarchical
\underline{T}ime-series),  a neural probabilistic \htsf method that
provides an end-to-end Bayesian approach to model the distributions of
forecasts of all time-series together (see Table \ref{tab:comp} for a comparison).
Specifically, we introduce a novel \textit{Soft Distributional Coherency Regularization (\sdcr)} to tackle the challenge \zc{you are introducing too many acronyms}  .
First, \sdcr enables \model to leverage hierarchical relations over entire forecast distributions
to generate calibrated forecast distributions by encouraging forecast distribution of any parent node to be similar to aggregation of children nodes' forecast distribution (Figure \ref{fig:start}).
Second, since \sdcr is a soft constraint, our model is trained to adapt to datasets with varying
hierarchical consistency that allows the model to trade-off coherency for better accuracy and calibration on weakly consistent datasets.
%\zc{too many points in this  sentence} .
%We compare the benefits of \model with previous methods in Table \ref{tab:comp}.
%\zc{need to better structure this paragraph of model design description}  
Our main contributions are: \\
\noindent\textbf{(1) Accurate and Calibrated Probabilistic Hierarchical Time-Series Forecasting:} We propose \model, a deep probabilistic framework for modeling the distributions of each time-series together using a soft distributional coherency regularization (\sdcr).
\model leverages probabilistic deep-learning models to learn priors of individual time-series and refines the priors of all time-series leveraging the hierarchy to provide accurate and well-calibrated forecasts.\\
\textbf{(2) Adaptation to Strong and Weak Consistency  via Soft Distributional Coherency Regularization:} \sdcr  imposes soft hierarchical constraints on the full forecast distributions to  help adapt the model to varying levels of hierarchical consistency.
We build a novel refinement module over raw forecast priors and leverage multi-task learning over shared parameters that enable \model to perform consistently well across the hierarchy.\\
%Our design choices also allows \model to automatically learn, for each time-series, a good trade-off between leveraging information from entire hierarchy and past patterns of time-series Thus \model automatically adapts  to different levels of strictness of coherency across benchmarks.\\
\textbf{(3) Evaluation Across Multiple Datasets and with Missing Data:} We show that our method \model outperforms a wide variety of state-of-the-art baselines on both accuracy and calibration, at all levels of the hierarchy, for both strong and weakly consistent datasets.
We also show training using \sdcr enables \model to leverage hierarchical relations to provide reliable predictions that can handle missing data values in the time-series. %Finally, we empirically observe the merits of our design choices through a detailed ablation study.

% \zc{table not referred in the text?} 




==> Text/method_old.tex <==
\section{Methodology}
\begin{figure*}[!thb]
    \centering
    \includegraphics[width=.98\linewidth]{Images/Main3.pdf}
    \caption{Overview of pipeline of \model. The input time series is ingested by \camul, a Neural Gaussian Process based probabilistic forecasting model to output the  raw forecast distribution. The parameters of raw forecasts are refined by the Refinement module using predictions from all time-series. The training is driven by a likelihood loss that learns from ground truth  and Soft Distributional Coherency Regularization that regularizes the forecast distribution to follow the hierarchical relations.}
    \label{fig:main}
\end{figure*}
\paragraph{Overview}
\model models the forecast distributions $\{P(y_{i}^{(t+\tau)}|\mathcal{D}^t)\}_{i=1}^N$ of all time-series nodes of the hierarchy by leveraging the relations from the hierarchy to provide accurate and well-calibrated forecasts that are adaptable to varying hierarchical consistency.
Most existing methods do not attempt to model the entire probabilistic distribution but focus on the coherency of point forecasts
or samples or fixed quantiles of the distribution \citep{rangapuram2021end,han2021simultaneously}.
This approach does not fully capture the uncertainty of the forecasts and in turn, does not provide calibrated predictions.
Methods like \pembu, \mint and \erm are post-processing steps that do not allow the forecasting model to learn from
relations across the hierarchy.
Moreover, most methods assume that the datasets are strongly consistent over hierarchical relations.
However, many real-world datasets are weakly consistent with time-series values of all nodes of the hierarchy observed simultaneously
and may not follow the hierarchical relations strictly due to noise and discrepancies in collecting data at different levels.
Therefore, most previous works may not adapt well to such deviations from these constraints.% \alex{you are repeating things from the intro so you could state this sharper here}
%For instance, the projection operation used in \citep{rangapuram2021end} to convert incoherent forecasts to be exactly coherent are sensitive to perturbations from
%coherency.
%is not the case in some real-world applications where noise and other factors cause data to deviate from these assumptions. Thus, previous methods, that don't adapt to these deviations due to their hard constraints, are very sensitive to such perturbations.


\model, on the other hand, reconciles the need to model coherency between entire forecast distributions as well as induce a soft adaptable constraint to enforce coherency
via a two-step process that is trained in an end-to-end manner.
The first component of \model is a differentiable neural probabilistic model that
produces a \textit{raw forecast} distribution for each node parameterized by $\{(\basemu_i, \basesigma_i)\}_{i=1}^N$ by using past values of time-series.
Raw forecasts of all nodes are used as priors to derive a refined set of forecast distributions parameterized by $\{({\mu}_i, {\sigma}_i)\}_{i=1}^N$ via the \textit{refinement module}.
The full probabilistic process of \model is depicted in Figure \ref{fig:main}.
\hide{
    \begin{equation}
        \begin{split}
            &P(\{y_i^{(t+\tau)}\}_{i=1}^N| \mathcal{D}^t) =\\
            \int
            &\underbrace{P(\mathbf{z}|\{ \mathbf{y}_i^{(1:t)}\}_{i=1}^N) \left(\prod_{i=1}^{N} P(\mathbf{z}_i,\mathbf{u}_i|\{ \mathbf{y}_i^{(1:t)}\}_{i=1}^N) P(\basemu_i, \basesigma_i|\mathbf{z}_i, \mathbf{z}, \mathbf{u}_i) \right)}_{\text{\camul (Raw forecasts)}} \\
            &\underbrace{\prod_{i=1}^N P(\mu_i, \sigma_i| \{\basemu_j, \basesigma_j\}_{j=1}^N) P(y_i^{(t+\tau)}|\mu_i, \sigma_i)}_{\text{Refinement Module}} d\{\mathbf{u}_i\}_{i=1}^N d\{\mathbf{z}_i\}_{i=1}^N.
        \end{split}
        \label{eqn:process}
    \end{equation}
}
% where $\mathbf{z}_i, \mathbf{u}_i, \mathbf{z}$ are intermediate latent variables of our probabilistic raw forecasting model TSFNP (Section \ref{sec:ngp}).
%\alex{we have space below each equation, it would be easier to understand for the reader if we specify what TSFNP is. in fact, TSFNP hasn't been introduced?}
\model's \sdcr regularizes the parameters $\{(\mu_i, \sigma_i)\}_{i=1}^N$ to leverage the hierarchical relations by minimizing the Distributional Coherency Error (DCE) defined as follows:
\begin{definition}(Distributional Coherency Error - DCE)
    Given the forecasts at time $t+\tau$ as $\{p_M(y_1^{(t+\tau)}|\mathcal{D}^t),\dots p_M(y_N^{(t+\tau)}|\mathcal{D}^t)\}$ distributional coherency error (DCE) is defined as
        {
            \begin{equation}
                \sum_{i\in \{1,\dots,N\}, \mathcal{C}_i\neq \emptyset} Dist\left(p_M(y_i^{(t+\tau)}|\mathcal{D}^t), p_M(\sum_{j\in \mathcal{C}_i} \phi_{i,j} y_j^{(t+\tau)}|\mathcal{D}^t) \right)
            \end{equation}
        }
    where $Dist$ is a distributional distance metric.
\end{definition}
Leveraging distributional coherency error as a soft regularizer enforces forecast distributions to be well-calibrated while adaptively adhering to hierarchical relations of the dataset.

%We describe the raw forecasting model \camul in Section \ref{sec:ngp}.

%1) \camul Raw Forecast (Section \ref{sec:ngp}): We first use a state-of-the-art Neural Gaussian Process (NGP) based time-series deep probabilistic forecasting model \camul to generate distribution parameters for the \textit{raw forecasts} for each of the time-series using past values of each time-series. 2) Refinement Module (Section \ref{sec:refinement}): The generated \textit{raw forecast distributions} serve as priors from which we derive the parameters of the \textit{refined forecast} distribution via the Coherency-based \textit{Refinement Module} by leveraging hierarchical relations via soft regularization. Each time-series' \textit{refined forecast} distribution is derived from \textit{raw forecast} distribution of \textit{all} time-series. Thus the \textit{refined forecasts} are learned by leveraging input data from all time-series.
%The training losses of the \model is applied on \textit{refined forecast} distribution to optimize for both forecast performance and coherency of the distributions (Section \ref{sec:loss}).

\subsection{Raw forecast distributions from NGPs}
\label{sec:ngp}
%NGPs combines the flexibility of non-parametric Gaussian Process based Functional Neural Process \citep{louizos2019functional} and the representative power of deep sequential models to provide accurate and well-calibrated predictions. 
%\zc{First time occurrence of NGP, spell out the full name. }
NGPs (Neural Gaussian Process) \citep{louizos2019functional}
are novel class of probabilistic neural models state-of-the-art accurate and calibrated predictions.
We, therefore, use a modified form of a state-of-the-art NGP model for time-series forecasting \citep{kamarthi2021doubt} which we call \camul to derive raw forecast distributions for each time-series.

We briefly describe \camul's  three components:
1) \textit{Probabilistic Neural Encoder}: It encodes the input univariate time-series into a latent stochastic embedding via a GRU \citep{cho2014properties} followed by a self-attention layer \citep{vaswani2017attention}:
{\begin{equation}
    \begin{split}
        [\mathbf{\mu}_{\mathbf{u}_i}, \log \sigma_{\mathbf{u}_i}] &= \text{Self-Atten}(\text{GRU}(\mathbf{y}_i^{(t':t)})),\\
        \mathbf{u}_i &\sim \mathcal{N}(\mathbf{\mu}_{\mathbf{u}_i}, \sigma_{\mathbf{u}_i}).
    \end{split}
\end{equation}}
2) \textit{Stochastic Data Correlation Graph}: We further leverage similar patterns of past time-series data and aggregate them as \textbf{local latent variable}. Unlike \epifnp which uses past time-series information from same node, in our multi-variate case \camul uses past information from all nodes. Formally, for input sequence $\mathbf{y}_i^{(t':t)}$ and each of the past sequence $\mathbf{y}_j$ where $j \in \{1, \dots, N\}$, we sample $\mathbf{y_j}$  with probability $\exp(-\gamma||\mathbf{u}_i-\mathbf{u}_j||_2^2)$ into set $N_i$. Then, we derive the local latent variable as
    {\begin{equation}
            \mathbf{z}_i \sim \mathcal{N}\left( \sum_{j\in N_i}\Theta_1(\mathbf{u}_j), \exp(\sum_{j\in N_i}\Theta_2(\mathbf{u}_j)) \right)
        \end{equation}}
where $\Theta_1$ and $\Theta_2$ are feed-forward networks.

3) \textit{Predictive Distribution Decoder}: Finally, we combine the latent embedding of input time-series, local latent variable and combined information of all past sequences to derive the parameters of the output distribution via a simple feed-forward network. We first derive a \textit{global latent variable} that combines the information from latent embeddings of all past sequences  as $\mathbf{z} = \sum_{i=1}^N \beta_i \mathbf{u}_i$ where the attention weights are $\{\beta_i\}_{i=1}^N$ are derived via self-attention as $\{\beta_i\}_{i=1}^N = \text{Self-Atten}(\{\mathbf{u}_i\}_{i=1}^N)$.

Finally, we combine the latent embedding of input time-series, local latent variable and global latent variable to derive the raw forecast distribution modelled as a Gaussian $\mathcal{N}(\basemu_i, \basesigma_i)$ as:
{\begin{equation}
    \begin{split}
        \mathbf{e} = \text{concat}(\mathbf{u}_i, \mathbf{z}_i, \mathbf{z}), \quad
        [\basemu_i, \log \basesigma_i] = \Theta_3(\mathbf{e})
    \end{split}
\end{equation}}
where $\Theta_3$ is a feed forward network.
\subsection{Refinement module}
\label{sec:refinement}
The refinement module leverages the raw distributions of all nodes of hierarchy to produce refined forecast distributions using hierarchical relations.
Given the parameters of \textit{raw forecast} distributions $\{\basemu_i, \basesigma_i\}_{i=1}^N$ derived from \camul for all time-series $\{\mathbf{y}_i^{(t':t)}\}_{i=1}^N$, the refinement module derives
the refined forecast distributions denoted by parameters $\{\mu_i, \sigma_i\}_{i=1}^N$ as functions of parameters of raw forecasts of all time-series.
The refined forecasts are optimized to be more coherent using \sdcr. Since we drive the full distributions of refined forecasts to be coherent, rather than just the samples or mean statistics, the refined distributions' calibration is also consistent with the hierarchical relations.


Let $\hat{\mathbf{\mu}} = [\basemu_{1} \dots, \basemu_N]$ and $\mathbf{\basesigma} = [\basesigma_{1} \dots, \basesigma_N]$ be vectors of means and standard deviations of raw distributions.
We model the refined mean as a function of the raw means of all the nodes.
Formally, we derive the mean $\mu_i$ of refined distribution as a weighted sum of two terms: a) $\basemu_i$, the mean of raw time-series, and b) linear combination of all raw mean of all time-series:
{\begin{equation}
    \gamma_i = \text{sigmoid}(\hat{w}_i), \quad
    \mu_i = \gamma_i \hat{\mu_i} + (1-\gamma_i) \mathbf{w}_i^T\basemu.
    \label{eqn:corem1}
\end{equation}}
$\{\hat{w}_i\}_{i=1}^N$ and $\{\mathbf{w}_{i}\}_{i=1:N}$ are both learnable set of parameters of the model. $\text{sigmoid}(\cdot)$ denotes the sigmoid function.  $\gamma_i$ helps model the trade-off between the influence of the raw distribution of node $i$ and the influence of the other nodes of the hierarchy. This is useful for the model to automatically adapt to datasets with varying hierarchical consistency.

Similarly, we assume the variance of the refined distribution depends on the raw mean and variance of all the time-series.
The variance parameter $\sigma_i$ of the refined distribution is derived from the raw distribution parameters $\mathbf{\basemu}$ and $\mathbf{\basesigma}$ as
    {\begin{equation}
            \sigma_i = c\hat{\sigma_i} \text{sigmoid}(\mathbf{v}_{1i}^T\mathbf{\basemu} + \mathbf{v}_{2i}^T \mathbf{\basesigma} + b_i)
            \label{eqn:corem2}
        \end{equation}}
where $\{\mathbf{v}_{1i}\}_{i=1}^N$, $\{\mathbf{v}_{2i}\}_{i=1}^N$ and $\{b_i\}_{i=1}^N$ are parameters and $c$ is a positive constant hyperparameter.
\subsection{Likelihood Loss and Regularization over Hierarchy}
\label{sec:loss}
We optimize the probabilistic process of Equation \ref{eqn:process} for accuracy and calibration by leveraging hierarchical relations by training on likelihood loss on ground truth training data as well as \sdcr.
\paragraph{Likelihood Loss}
To maximise the likelihood of forecasts over ground truth $ P(\{y_i^{(t+\tau)}\}_{i=1}^N| \mathcal{D}_t)$ we use variational inference by approximating the posterior $P(\{\mathbf{u}_i, \mathbf{z}_i, N_i\}_{i=1}^N| \{y_i^{(t+\tau)}\}_{i=1}^N)$ with the variational distribution
\begin{equation}
    \begin{split}
        Q(\{\mathbf{u}_i, \mathbf{z}_i, N_i\}_{i=1}^N| \{y_i^{(t+\tau)}\}_{i=1}^N) &= P(\{\mathbf{u}_i, N_i\}_{i=1}^N| \{y_i^{(t+\tau)}\}_{i=1}^N)\\
        &\prod_{i=1}^N q_i(\mathbf{z}_i | \mathbf{y}_i^{(t':t)})
    \end{split}
\end{equation}
where $q_i$ is a feed-forward network over GRU hidden embeddings of Probabilistic Neural Encoder  that parameterizes the Gaussian distribution of $q_i(\mathbf{u}_i | \mathbf{y}_i^{(t':t)})$. We derive the ELBO (detailed derivation in Appendix) as
    {\begin{equation}
            \begin{split}
                \mathcal{L}_{1} =& -E_{Q(\{\mathbf{u}_i, \mathbf{z}_i, N_i\}_{i=1}^N, \mathbf{z}| \{y_i^{(t+\tau)}\}_{i=1}^N)} [\log P(\{y_i^{(t+\tau)}\}_{i=1}^N| \{\mathbf{u}_i, \mathbf{z}_i, N_i\}_{i=1}^N)\\
                &+ \sum_{i=1}^N \log P(\mathbf{z}_i | \{\mathbf{u}_j\}_{j=1}^N, N_i) - \log q_i(\mathbf{z}_i | \mathbf{y}_i^{(t':t)})].
            \end{split}
            \label{eqn:loss1}
        \end{equation}}
\paragraph{Soft Distributional Coherency Regularization}
\model leverages the hierarchy relations in $\mathcal{T}$ and regularizes the refined  distributions to be coherent.
Since \model aims to leverage hierarchical coherency for improved robustness and calibration, we regularize over the full distributions
by using \textit{distributional coherency error} as part of the loss function.
We use the Jensen-Shannon Divergence \citep{endres2003new} (JSD) as the distance metric since it is a symmetric and bounded variant of the popularly used KL-Divergence distance and assumes closed form for many widely used distributions.
We derive the \textit{distributional coherency error} on $\{(\mu_i, \sigma_i)\}_{i=1}^N$ as
    {\begin{equation}
            \begin{split}
                &\mathcal{L}_2 = 2\left[\sum_{i=1}^N \text{JSD}\left(P(y_i^{(t+\tau)}|\mu_i, \sigma_i), P\left(\sum_{j\in \mathbf{C}_i}\phi_{ij} y_j^{(t+\tau)}| \{\mu_j, \sigma_j\}_{j\in \mathbf{C}_i} \right)\right) + 1\right].
            \end{split}
            \label{eqn:jsd}
        \end{equation}}
Computation of JSD is generally intractable. However, in our case, due to parameterization
%\alex{before you used parameterize, be consistent} 
of each time-series distribution as a Gaussian we get a closed-form differentiable expression:
{\begin{equation}
    \begin{split}
        \mathcal{L}_2 &= \sum_{i=1}^N \frac{\sigma_i^2 + \left( \mu_i - \sum_{j\in C_i} \phi_{ij}\mu_j \right)^2}{2\sum_{j\in C_i}\phi^2_{ij} \sigma_j^2} +\\
        &\sum_{i=1}^N  \frac{\sum_{j\in C_i}\phi^2_{ij} \sigma_j^2 + \left( \mu_i - \sum_{j\in C_i} \phi_{ij}\mu_j \right)^2}{2\sigma_i^2} .
    \end{split}
    \label{eqn:jsd2}
\end{equation}}


We provide the derivation of Equation \ref{eqn:jsd2} in the Appendix.
We use the distributional coherency error as a soft regularization term to enable  \model to leverage constraints $H_\mathcal{T}$ when generating forecast distributions.
% unlike recent probabilistic methods \citep{rangapuram2021end} that regularizes over individual samples.
%, we regularize for coherency over the entire distribution accounting for modelling both coherent mean statistics as well as calibration of refined distribution leading to more robust modelling of forecasts.
Thus, the total loss for training is given as
$\mathcal{L} = \mathcal{L}_1 + \lambda \mathcal{L}_2$
where the hyperparameter $\lambda$ controls the trade off between data likelihood and coherency.
%Tuning $\lambda$ also allows \model to adapt to datasets of different levels of adherence \alex{adherence should be coherency? or is it something else? adherence was never defined} to aggregation function of proposed hierarchy (unlike \citep{rangapuram2021end} that assumes strict adherence).
We also use the reparameterization trick to make the sampling process differentiable and we learn the parameters of all training modules via Stochastic Variational Bayes \citep{kingma2013auto}. The full pipeline of \model is summarized in Figure \ref{fig:main}.

\subsection{Details on Training}
\label{sec:train_steps}
%We provide additional important details for effective training of \model here. 
\noindent\textbf{Parameter sharing across nodes}
Since \model's \camul module forecasts for multiple nodes, we leverage the hard-parameter sharing paradigm of multi-task learning \citep{caruana1997multitask} and use different set of parameters for Predictive Distribution Decoder (i.e., weights of $\Theta_3$) whereas the parameters of other components of \camul are shared across all nodes (Figure \ref{fig:main}). Sharing parameters for Probabilistic Neural Encoder drastically lowers the number of learnable parameters since datasets can have large number of nodes (up to 512 nodes in our experiments).% Since we share the weights of Probabilistic Neural Encoder, we also project the latent embeddings of input time-series of all nodes to same latent space for generating Stochastic Correlation Graph.

\noindent\textbf{Pre-training on individual time-series}
Before we start training for refined forecasts, we  pre-train the parameters of \camul on given training dataset to model raw forecast distribution accurately. We train using only a log likelihood loss to learn parameters $\{\basemu_i, \basesigma_i\}_{i=1}^N$ similar to Equation \ref{eqn:loss1}.




==> Text/results_dump.tex <==
\subsection{Results}
We comprehensively understand the efficacy of \model by evaluating it through the following questions:
\begin{enumerate}[label={(\bfseries Q\arabic*):}]
    \item  Does \model predict accurate calibrated forecasts across all benchmarks?
    \item Does \model provide consistently better performance across all levels of the hierarchy?
    \item Does \model provide robust accurate forecasts if input sequences have missing data?
    \item Does \model adapt to different strictness of coherency in datasets?
%    \item How does various design choices of \model contribute to its performance, robustness and adaptability?
\end{enumerate}

\subsubsection{Accuracy and Calibration performance (Q1)}
\input{Text/table_all}
We evaluate  all baselines, \model and its variants for the datasets described in Section \ref{sec:expt} over 5 independent runs. We report the average CRPS and IS scores across all levels hierarchy in Table \ref{tab:tab1}. We observe that \model significantly outperforms all baselines in CRPS score by 41\%-88\% and IS by 14\%-550\%. 
%Specifically, for strongly-coherent benchmarks we see an average improvement of 54\% in CRPS. We observe a large 93\% average improvement in weakly-coherent benchmarks. 
Thus, \model adapts well to varied kinds of datasets and outperforms all baselines. Performing t-test with significance $\alpha=1\%$ we find the all the scores are statistically significant compared to baselines. Therefore, \model outperforms previous state-of-art models in both accuracy and calibration overall benchmarks.

On comparing the performance of \model with the variants, we observe that \model comparable to or better than best performing variant in each dataset

\subsubsection{Performance across the hierarchy (Q2)} 

Next we look at performance of all models across each level of hierarchy.
We compare the performance of \model with best performing baselines \hiere and \sharq for all datasets in Table \ref{tab:levels}.
Again we observe that \model significantly outperforms the best baselines. At the leaf nodes, which contains most data, \model outperforms best baselines by 7\% in \wiki to 100\% in \fbsymp. For the top node of time-series the performance improvement is larges at 35\% (\wiki) to 962\% (\fbsymp).
%On performing t-test for each level of hierarchy we gain found these improvements to be statistically significant.
%



\input{Text/table_levels}



\subsubsection{Robust forecasting through data imputation (Q3)}

\input{Text/table_miss}

During real-time forecasting in real world applications such as Epidemic or Sales forecasting, we encounter situations where past few values of time-series are missing or unreliable for some of the nodes, specifically at lower levels, due to discrepancies during reporting and other factors \cite{chakraborty2018know}.
Therefore, one approach to perform forecasting in such situation is first by imputation of missing values based on past data and then using the predicted missing values as part of the input for forecasting. \textbf{Task:} To simulate such scenarios to evaluate robustness of \model, we propose the task of \textit{Hierarchical Forecasting with missing values} (HFMV). Formally, at time-period $t$, we are given full data for upto time $t'<t$ (we set $t'=t-5$) and for sequence values in time period between $t'$ and $t$, we remove these values from dataset with probability $p$. The goal of HFMV is to use the given partial dataset from $t'$ to $t$ as input to predict future values at $t+\tau$.

\textbf{Setup:}
We first train \model on complete dataset till time $t'$ and then fill in the missing values of input sequence using the trained model. Using the predicted missing values, we again forecast the output distribution. Since \model is probabilistic, we perform multiple iterations of sampling for missing values followed by forecasting future values. We estimate the evaluation scores using sample forecasts from all sampling iterations.

\textbf{Result:}
We compare the performance of \model with \hiere, the top baseline that uses coherency and vanilla \camul which that doesn't use coherency. We measure relative decrease in performance with increase in probability $p$ (Figure \ref{fig:miss1}). We observe that \model's performance decrease with larger probability of missing values is much slower compared to other baselines. Even at $p=0.1$, \model's performance decreases by 10.45-26.8\% compared to other baselines that consistently decrease by over 70\%.
Thus, \model effectively leverages coherency to model missing values.

\subsubsection{Adaptability of \model to perturbation of coherency (Q4)}

The hierarchical relations in dataset like \tourism, \labour and \wiki are synthetically constructed while pre-processing the data i.e., the time-series of only the leaf nodes are collected and the
values of time-series of other nodes of hierarchy are generated using the hierarchical relations.
Therefore, these datasets strictly follow the hierarchical relations and we denote them as \textit{strongly coherent}.
For other real-world datasets like \symp and \fbsymp, the values of all nodes of hierarchy
are directly collected or measured and not generated by modellers through aggregation. 
Therefore, they contain values in time-series that may deviate from the postulated hierarchical relations, especially at leaf nodes due to many factors like measurement noise, reporting errors,
asynchronous data revisions, etc \cite{chakraborty2018know}. We call these datasets \textit{weakly coherent}.

Since most previous state-of-art models assume datasets to be strictly coherent, small perturbations
to this assumptions can cause large errors and under-performance when used with weakly coherent data.
In contrast, the design choices of Refinement Module and soft regularization of distributional coherency loss enables \model to adapt to datasets of different strictness of coherency. 
Specifically, by optimizing for values of $\{\gamma_i\}_{i=1}^N$ of Equation \ref{eqn:corem1}, \model automatically learns a good trade-off between leveraging prior forecasts fo a time-series and forecasts entire hierarchy.


Looking at performance benchmarks in Table \ref{tab:tab1}, while \model provides 54\% in CRPS for strongly-coherent datasets, we observe a much larger 93\% average improvement for weakly-coherent case.
Similarly, we also see larger differences in scores at each level of hierarchy for weakly-coherent datasets in Table \ref{tab:levels}. 

%We also observe that for both strongly and weakly coherent datasets at lower levels of hierarchy \model has larger improvements in performance (32\%-165\% improvement in CRPS). This is because the nodes at lower level show more complex patterns. Therefore, apart from learning from past patterns of time-series, \model effectively leverages information from other nodes of hierarchy to better estimate these values. Since \model can adapt to these discrepancies in hierarchical relations due to soft regularization via distributional coherency loss, \model also our-performs other more strictly constrained baselines for weakly coherent datasets. Some of the leaf-nodes of weakly coherent datasets have values that show larger deviations from hierarchical relations. While this phenomenon will destabilise the forecasts of models like \cite{rangapuram2021end} that enforce projection of forecasts to space of strict coherence, \model can adapt to such changes without perturb values of other time-series too much.


We also study the learned values of $\{\gamma_i\}_{i=1}^N$ of Equation \ref{eqn:corem1} used to derive refined mean. Note that higher values of $\gamma_i$ indicate larger dependence on raw forecasts of node and smaller dependence of forecasts of entire hierarchy.
We plot the average values of $\gamma_i$ for each of the datasets in Table \ref{tab:gamma}. We observe that strongly coherent datasets have lower values of $\gamma_i$ indicating that \model automatically learns to strongly leverage the hierarchy for these datasets compared to weakly coherent datasets.
\iffalse
\begin{figure}[h]
    \centering
    \includegraphics[width=.6\linewidth]{Images/gamma1_1.pdf}
    \caption{Average value of $\gamma_i$ for all datasets. Note that weakly coherent datasets have higher $\gamma_i$ (depends mode on past data of same time-series) where as strongly-coherent data have lower $\gamma_i$ (leverages the hierarchical relations).}
    \label{fig:gamma}
\end{figure}
\fi

\begin{table}[h]
\caption{Average value of $\gamma_i$ for all datasets. Note that weakly coherent datasets have higher $\gamma_i$ (depends mode on past data of same time-series) where as strongly-coherent data have lower $\gamma_i$ (leverages the hierarchical relations).}
\centering
\begin{tabular}{c|cc}
Consistency & Dataset   & \multicolumn{1}{l}{Mean $\gamma_i$} \\ \hline
Strong    & Tourism-L & 0.420  $\pm$ 0.096                                        \\
          & Labour    & 0.348  $\pm$ 0.091                                        \\
          & Wiki      & 0.313  $\pm$ 0.057                                        \\ \hline
Weak      & Symp      & 0.759  $\pm$ 0.152                                        \\
          & Fbsymp    & 0.789  $\pm$ 0.180                                       
\end{tabular}
\label{tab:gamma}
\end{table}

\subsubsection{Ablation Studies (Q6)}

We study the impact of various modelling choices of \model towards its forecasting performance, adaptability and robustness through the following ablation study.
\noindent\textit{\model Variants:} We introduce the following variants of \model to evaluate the importance of different components of \model.
    $\bullet$\textbf{P-Global:} We study the effect of of our multi-tasking hard-parameter sharing approach (Section\ref{sec:train_steps}) by training a variant where all the parameters, including PDD are shared across all the nodes.
$\bullet$\textbf{P-FineTune:} We also look at the efficacy of our soft reguliarization using both losses (Equation \ref{eqn:loss}) that adapts to optimize for both coherency and training accuracy by comparing it with a variant where the PDD parameters are further fine-tuned for individual nodes using only the likelihood loss.
$\bullet$\textbf{P-DeepVAR:} We evaluate our choice of using \camul, a previous state-of-art univariate forecasting model for accurate and calibrated forecasts with DeepVAR \cite{salinas2020deepar}, another popular probabilistic forecasting model that was also used in \hiere baseline \cite{rangapuram2021end}.
$\bullet$\textbf{P-noCoherent:} This variant is trained by completely removing the distributional coherency loss from training. Note that unlike P-FineTune which was initially trained with coherency loss before fine-tuning,  P-noCoherent never uses the coherency loss at any point of training routine. Therefore P-noCoherent measures the importance of explicitly regularizing over the information from hierarchy.


\paragraph{Performance comparison with variants:}

%\input{Text/table_var}
We compare the performance of variants in Table \ref{tab:tab1}. First, we observe that the performance of \model is almost always comparable to or better than all other variants. We observe that P-Global has similar performance to \model in strongly coherent datasets where the coherency relations are captures by the global set of parameters for all time-series. We also see that P-NoCoherent's performance is also significantly worse for strongly-coherent datasets. In contrast, P-FineTune has similar or slightly better performance to \model in weakly coherent datasets byut P-Global's performance is very poor. Thus, \model is a overall better model applicable to both kinds of datasets. Finally, using DeepVAR over \camul for raw forecasts, doesn'y improve performance in any of the datasets.

%\input{Text/table_levels_var}
Looking at level-wise CRPS score in Table \ref{tab:levels}, we observe that \model consistently performs better than all variants in most higher levels. P-Global's performance in strongly coherent datasets is due to its performance in last level of hierarchy. Similarly for P-FineTune in case of weakly-coherent datasets.

\paragraph{Performance of variants under missing data (HFMV)}
\input{Text/table_miss2}

We measure the \% performance decrease of all variants with increase in proportion of missing data in the HFMV task. We observe that P-NoCoherent's performance deteriorates very rapidly in most benchmarks, showing the importance of distributional coherency loss for learning provide robust calibrated coherent forecasts. We also observe that \model and P-Global suffers least degradation in performance since both these models prioritize integrating hierarchical coherency information which enables them to provide better estimates for imputed data for missing input and use them generate more accurate and calibrated forecasts.





\subsubsection{Ablation Studies (Q6)}


\paragraph{Performance comparison with variants:}

%\input{Text/table_var}
We compare the performance of variants in Table \ref{tab:tab1}. First, we observe that the performance of \model is almost always comparable to or better than all other variants. We observe that P-Global has similar performance to \model in strongly coherent datasets where the coherency relations are captures by the global set of parameters for all time-series. We also see that P-NoCoherent's performance is also significantly worse for strongly-coherent datasets. In contrast, P-FineTune has similar or slightly better performance to \model in weakly coherent datasets byut P-Global's performance is very poor. Thus, \model is a overall better model applicable to both kinds of datasets. Finally, using DeepVAR over \camul for raw forecasts, doesn'y improve performance in any of the datasets.

%\input{Text/table_levels_var}
Looking at level-wise CRPS score in Table \ref{tab:levels}, we observe that \model consistently performs better than all variants in most higher levels. P-Global's performance in strongly coherent datasets is due to its performance in last level of hierarchy. Similarly for P-FineTune in case of weakly-coherent datasets.

\paragraph{Performance of variants under missing data (HFMV)}

We measure the \% performance decrease of all variants with increase in proportion of missing data in the HFMV task. We observe that P-NoCoherent's performance deteriorates very rapidly in most benchmarks, showing the importance of distributional coherency loss for learning provide robust calibrated coherent forecasts. We also observe that \model and P-Global suffers least degradation in performance since both these models prioritize integrating hierarchical coherency information which enables them to provide better estimates for imputed data for missing input and use them generate more accurate and calibrated forecasts.



==> Text/table_all.tex <==
\begin{table*}[h]
\caption{\textit{Average scores (accros 5 runs) on \textbf{strongly consistent} datasets across all levels for all baselines, \model and its variants. 
%\model significantly outperforms baselines (t-test with $\alpha=1\%$) with 54\% better CRPS and 20\% better calibration score.
}}
\label{tab/tab1}
\centering
\scalebox{0.65}{
\begin{tabular}{c|ccccc|ccccc|ccccc}
             &               &               & Tourism-L     &               &                &                &                & Labour        &               &               &                &                & Wiki          &               &               \\ \hline
Models/Data  & MAPE\%        & CRPS          & LS            & CS            & DCE            & MAPE\%         & CRPS           & LS            & CS            & DCE           & MAPE\%         & CRPS           & LS            & CS            & DCE           \\ \hline
DeepVAR      & 3.12          & 0.17          & 0.61          & 0.19          & 0.32           & 18.27          & 0.045          & 0.75          & 0.25          & 0.34          & 16.52          & 0.232          & 0.83          & 0.27          & 0.26          \\
EpiFNP       & 2.28          & 0.21          & 1.19          & 0.14          & 0.39           & 14.52          & 0.071          & 1.41          & 0.21          & 0.22          & 15.63          & 0.287          & 0.86          & 0.21          & 0.39          \\
TSFNP-MinT   & 1.17          & 0.5           & 0.58          & 0.15          & 0.24           & 16.46          & 0.045          & 4.12          & 0.26          & 0.12          & 13.79          & 0.243          & 0.78          & 0.18          & 0.18          \\
TSFNP-ERM    & \textbf{1.42} & 0.56          & 0.53          & 0.11          & 0.18           & 13.57          & 0.045          & 3.63          & 0.23          & 0.19          & 17.74          & 0.221          & 0.74          & 0.19          & 0.21          \\
HeirE2E      & 1.67          & 0.15          & 0.38          & 0.17          & 0.21           & \textbf{12.53} & 0.034          & 0.51          & 0.25          & 0.15          & 17.05          & 0.211          & 0.46          & 0.23          & 0.12          \\
SHARQ        & 1.63          & 0.17          & 0.41          & 0.12          & 0.13           & 14.21          & 0.054          & 0.47          & 0.18          & 0.09          & 16.13          & 0.241          & 0.52          & 0.16          & 0.16          \\
PEMBU-MinT   & 1.77          & 0.15          & 0.46          & 0.24          & 0.03           & 13.55          & 0.039          & 0.56          & 0.22          & 0.11          & 14.66          & 0.279          & 0.58          & 0.21          & 0.05          \\
PEMBU-ERM    & 1.63          & 0.16          & 0.43          & 0.21          & \textbf{0.02}  & 13.19          & 0.042          & 0.61          & 0.25          & \textbf{0.03} & 15.79          & 0.268          & 0.54          & 0.18          & 0.02          \\ \hline
ProfHit      & 1.47          & \textbf{0.12} & \textbf{0.33} & \textbf{0.09} & \textbf{0.02}  & 12.79          & \textbf{0.026} & \textbf{0.21} & \textbf{0.14} & 0.05          & \textbf{12.47} & \textbf{0.184} & \textbf{0.35} & \textbf{0.13} & \textbf{0.04} \\ \hline
P-FineTune   & 1.52          & 0.16          & 0.39          & 0.14          & 0.25           & 14.36          & 0.031          & 0.36          & 0.21          & 0.13          & 13.22          & 0.216          & 0.39          & 0.21          & 0.08          \\
P-Global     & 1.47          & 0.13          & 0.42          & \textbf{0.06} & \textbf{0.01}  & \textbf{12.17} & 0.027          & 0.31          & 0.16          & 0.04          & \textbf{12.37} & 0.185          & 0.34          & 0.16          & 0.04          \\
P-DeepAR     & \textbf{1.45} & 0.13          & 0.52          & 0.12          & 0.04           & 13.44          & 0.029          & 0.58          & 0.17          & 0.08          & 12.89          & 0.201          & 0.48          & 0.24          & 0.07          \\
P-NoCoherent & 1.82          & 0.18          & 0.37          & 0.21          & 0.35           & 16.97          & 0.043          & 0.45          & 0.26          & 0.17          & 17.44          & 0.227          & 0.47          & 0.35          & 0.14                 
\end{tabular}
}
\end{table*}
\begin{table*}[h]
\caption{\textit{Average scores (accros 5 runs) on \textbf{weakly consistent} datasets across all levels for all baselines, \model and its variants. 
%\model significantly outperforms baselines (t-test with $\alpha=1\%$) with 25-52\% better accuracy and 37\% better calibration.
}}
\label{tab/tab1_1}
\centering
\scalebox{0.65}{
\begin{tabular}{c|ccccc|ccccc}
             &        &                & Flu           &                &               &        &               & FB Symptoms   &               &               \\ \hline
Models/Data  & MAPE\% & CRPS           & LS            & CS             & DCE           & MAPE\% & CRPS          & LS            & CS            & DCE           \\ \hline
DeepVAR      & 31.27  & 0.610          & 3.25          & 0.065          & 0.31          & 17.39  & 7.32          & 5.32          & 0.17          & 0.29          \\
EpiFNP       & 12.8   & 0.460          & 0.93          & 0.034          & 0.42          & 15.35  & 5.53          & 7.84          & 0.11          & 0.37          \\
TSFNP-MinT   & 10.56  & 0.630          & 3.18          & 0.082          & 0.18          & 12.24  & 5.39          & 6.35          & 0.14          & 0.24          \\
TSFNP-ERM    & 11.85  & 0.620          & 2.75          & 0.075          & 0.12          & 13.16  & 6.14          & 4.23          & 0.12          & 0.19          \\
HeirE2E      & 15.67  & 0.420          & 0.81          & 0.12           & 0.32          & 12.63  & 4.12          & 1.13          & 0.19          & 0.26          \\
SHARQ        & 18.34  & 0.470          & 1.42          & 0.071          & 0.21          & 12.82  & 3.12          & 0.81          & 0.15          & 0.19          \\
PEMBU-MinT   & 15.44  & 0.621          & 2.55          & 0.18           & \textbf{0.05} & 13.75  & 5.78          & 4.22          & 0.22          & \textbf{0.07} \\
PEMBU-ERM    & 17.57  & 0.688          & 2.74          & 0.15           & 0.07          & 12.99  & 6.31          & 5.18          & 0.18          & 0.1           \\ \hline
ProfHit      & 8.85   & \textbf{0.250} & \textbf{0.28} & \textbf{0.042} & 0.14          & 9.67   & \textbf{1.43} & \textbf{0.45} & \textbf{0.08} & 0.16          \\ \hline
P-FineTune   & 10.44  & 0.240          & 0.3           & \textbf{0.039} & 0.17          & 9.83   & 1.18          & 0.72          & \textbf{0.07} & 0.19          \\
P-Global     & 14.27  & 0.350          & 0.47          & 0.086          & 0.09          & 12.11  & 2.64          & 1.39          & 0.14          & 0.11          \\
P-DeepAR     & 17.43  & 0.361          & 0.54          & 0.083          & 0.15          & 11.89  & 2.13          & 0.75          & 0.18          & 0.15          \\
P-NoCoherent & 9.17   & 0.248          & 0.36          & 0.16           & 0.22          & 13.99  & 1.17          & 0.84          & 0.24          & 0.22         
\end{tabular}
}
\end{table*}

==> Text/table_all3.tex <==
\begin{table*}[h]
\caption{Average scores (across 5 runs)  across all levels of hierarchy for all baselines, \model and its variants. 
\model provides 54\% better accuracy and 32\% better calibration. 
}
\label{tab:tab1}
%\centering
\scalebox{0.95}{
\begin{tabular}{@{}c@{}}
    \begin{minipage}{\textwidth}
    \centering
    \begin{tabular}{c|ccccc|ccccc|ccccc}
             &       \multicolumn{5}{c|}{\tourism} &    \multicolumn{5}{c|}{\labour} & \multicolumn{5}{c|}{\wiki}             \\ \hline
\textbf{Models/Data}  & \textbf{MAPE}\%        & \textbf{CRPS}          & \textbf{LS}            & \textbf{CS}            & \textbf{DCE}            & \textbf{MAPE}\%         & \textbf{CRPS}           & \textbf{LS}            & \textbf{CS}            & \textbf{DCE}           & \textbf{MAPE}\%         & \textbf{CRPS}           & \textbf{LS}            & \textbf{CS}            & \textbf{DCE}           \\ \hline
\deepvar      & 3.12          & 0.17          & 0.61          & 0.19          & 0.32           & 18.27          & 0.045          & 0.75          & 0.25          & 0.34          & 16.52          & 0.232          & 0.83          & 0.27          & 0.26          \\
\camul       & 2.28          & 0.21          & 1.19          & 0.14          & 0.39           & 14.52          & 0.071          & 1.41          & 0.21          & 0.22          & 15.63          & 0.287          & 0.86          & 0.21          & 0.39          \\
TSFNP-MinT   & 1.17          & 0.5           & 0.58          & 0.15          & 0.24           & 16.46          & 0.045          & 4.12          & 0.26          & 0.12          & 13.79          & 0.243          & 0.78          & 0.18          & 0.18          \\
TSFNP-ERM    & \textbf{1.42} & 0.56          & 0.53          & 0.11          & 0.18           & 13.57          & 0.045          & 3.63          & 0.23          & 0.19          & 17.74          & 0.221          & 0.74          & 0.19          & 0.21          \\
\hiere      & 1.67          & 0.15          & 0.38          & 0.17          & 0.21           & \textbf{12.53} & 0.034          & 0.51          & 0.25          & 0.15          & 17.05          & 0.211          & 0.46          & 0.23          & 0.12          \\
SHARQ        & 1.63          & 0.17          & 0.41          & 0.12          & 0.13           & 14.21          & 0.054          & 0.47          & 0.18          & 0.09          & 16.13          & 0.241          & 0.52          & 0.16          & 0.16          \\
PEMBU-\mint   & 1.77          & 0.15          & 0.46          & 0.24          & 0.03           & 13.55          & 0.039          & 0.56          & 0.22          & 0.11          & 14.66          & 0.279          & 0.58          & 0.21          & 0.05          \\
PEMBU-ERM    & 1.63          & 0.16          & 0.43          & 0.21          & \textbf{0.02}  & 13.19          & 0.042          & 0.61          & 0.25          & \textbf{0.03} & 15.79          & 0.268          & 0.54          & 0.18          & \textbf{0.02}          \\ \hline
\model      & 1.47          & \textbf{0.12} & \textbf{0.33} & \textbf{0.09} & \textbf{0.02}  & 12.79          & \textbf{0.026} & \textbf{0.21} & \textbf{0.14} & 0.05          & \textbf{12.47} & \textbf{0.184} & \textbf{0.35} & \textbf{0.13} & 0.04 \\ \hline
\finetune   & 1.52          & 0.16          & 0.39          & 0.14          & 0.25           & 14.36          & 0.031          & 0.36          & 0.21          & 0.13          & 13.22          & 0.216          & 0.39          & 0.21          & 0.08          \\
\pglobal     & 1.47          & 0.13          & 0.42          & \textbf{0.06} & \textbf{0.01}  & \textbf{12.17} & 0.027          & 0.31          & 0.16          & 0.04          & \textbf{12.37} & 0.185          & 0.34          & 0.16          & 0.04          \\
\pvar     & \textbf{1.45} & 0.13          & 0.52          & 0.12          & 0.04           & 13.44          & 0.029          & 0.58          & 0.17          & 0.08          & 12.89          & 0.201          & 0.48          & 0.24          & 0.07          \\
\nocoherent & 1.82          & 0.18          & 0.37          & 0.21          & 0.35           & 16.97          & 0.043          & 0.45          & 0.26          & 0.17          & 17.44          & 0.227          & 0.47          & 0.35          & 0.14                 
\end{tabular}
    \end{minipage}
    \\
    \begin{minipage}{\textwidth}
    \centering
    \begin{tabular}{c|ccccc|ccccc}
             &       \multicolumn{5}{c|}{\symp} &    \multicolumn{5}{c|}{\fbsymp}          \\ \hline
\textbf{Models/Data}  & \textbf{MAPE}\% & \textbf{CRPS}           & \textbf{LS}            & \textbf{CS}             & \textbf{DCE}           & \textbf{MAPE}\% & \textbf{CRPS}          & \textbf{LS}            & \textbf{CS}            & \textbf{DCE}           \\ \hline
\deepvar      & 31.27  & 0.610          & 3.25          & 0.065          & 0.31          & 17.39  & 7.32          & 5.32          & 0.17          & 0.29          \\
\camul       & 12.8   & 0.460          & 0.93          & 0.034          & 0.42          & 15.35  & 5.53          & 7.84          & 0.11          & 0.37          \\
TSFNP-\mint   & 10.56  & 0.630          & 3.18          & 0.082          & 0.18          & 12.24  & 5.39          & 6.35          & 0.14          & 0.24          \\
TSFNP-\erm    & 11.85  & 0.620          & 2.75          & 0.075          & 0.12          & 13.16  & 6.14          & 4.23          & 0.12          & 0.19          \\
\hiere      & 15.67  & 0.420          & 0.81          & 0.12           & 0.32          & 12.63  & 4.12          & 1.13          & 0.19          & 0.26          \\
SHARQ        & 18.34  & 0.470          & 1.42          & 0.071          & 0.21          & 12.82  & 3.12          & 0.81          & 0.15          & 0.19          \\
PEMBU-MinT   & 15.44  & 0.621          & 2.55          & 0.18           & \textbf{0.05} & 13.75  & 5.78          & 4.22          & 0.22          & \textbf{0.07} \\
PEMBU-ERM    & 17.57  & 0.688          & 2.74          & 0.15           & 0.07          & 12.99  & 6.31          & 5.18          & 0.18          & 0.1           \\ \hline
\model      & 8.85   & \textbf{0.250} & \textbf{0.28} & \textbf{0.042} & 0.14          & 9.67   & \textbf{1.43} & \textbf{0.45} & \textbf{0.08} & 0.16          \\ \hline
\finetune   & 10.44  & 0.240          & 0.3           & \textbf{0.039} & 0.17          & 9.83   & 1.18          & 0.72          & \textbf{0.07} & 0.19          \\
\pglobal     & 14.27  & 0.350          & 0.47          & 0.086          & 0.09          & 12.11  & 2.64          & 1.39          & 0.14          & 0.11          \\
\pvar     & 17.43  & 0.361          & 0.54          & 0.083          & 0.15          & 11.89  & 2.13          & 0.75          & 0.18          & 0.15          \\
\nocoherent & 9.17   & 0.248          & 0.36          & 0.16           & 0.22          & 13.99  & 1.17          & 0.84          & 0.24          & 0.22         
\end{tabular}
    \end{minipage}
    
\end{tabular}
}
\end{table*}


==> Text/table_levels_var.tex <==
\begin{table*}[h]
\centering
\begin{tabular}{c|cccccccccccc}
Models/Data          & \multicolumn{9}{c|}{Tourism-L}                                                                                                                                                                                        & \multicolumn{3}{c}{Labour}                       \\ \hline
 Hierarchy Levels               & 1              & 2              & 3              & 4              & 5                                   & 2(Geo)         & 3(Geo)         & 4(Geo)                              & \multicolumn{1}{c|}{1}              & 2              & 3              & 4              \\ \hline
\model-FineTune   & 0.072          & 0.136          & 0.083          & 0.16           & 0.278                               & 0.124          & 0.124          & 0.158                               & \multicolumn{1}{c|}{0.024}          & 0.022          & 0.026          & 0.035          \\
\model-Global     & 0.093          & 0.113          & 0.122          & 0.13           & \textbf{0.261}                      & 0.093          & 0.113          & 0.147                               & \multicolumn{1}{c|}{\textbf{0.021}} & 0.027          & 0.028          & \textbf{0.027} \\
\model-DeepVAR & 0.075          & 0.097          & 0.136          & 0.183          & 0.281                               & 0.095          & 0.122          & 0.159                               & \multicolumn{1}{c|}{0.025}          & 0.027          & 0.031          & 0.033          \\
\model-NoCoherent    & 0.086          & 0.142          & 0.107          & 0.18           & 0.265                               & 0.132          & 0.138          & 0.147                               & \multicolumn{1}{c|}{0.027}          & 0.031          & 0.029          & 0.026          \\ 
\model            & \textbf{0.051} & \textbf{0.095} & \textbf{0.12}  & \textbf{0.17}  & \textbf{0.264}                      & \textbf{0.083} & \textbf{0.106} & \textbf{0.142}                      & \multicolumn{1}{c|}{\textbf{0.023}} & \textbf{0.019} & \textbf{0.023} & 0.029          \\ \hline
 Models/Data              & \multicolumn{5}{c|}{Wiki}                                                                               & \multicolumn{3}{c|}{Flu-Symptoms}                                              & \multicolumn{3}{c}{FB Symptoms}                                       &                \\ \hline
  Hierarchy Levels               & 1              & 2              & 3              & 4              & \multicolumn{1}{c|}{5}              & 1              & 2              & \multicolumn{1}{c|}{3}              & 1                                   & 2              & 3              &                \\ \hline
\model-FineTune   &0.034          & 0.086          & 0.153          & 0.232          & \multicolumn{1}{c|}{0.275} & 0.222          & 0.175          & \multicolumn{1}{c|}{\textbf{0.293}} & 0.43                                & 0.65           & \textbf{1.83}  &                \\
\model-Global     &  0.048          & 0.103          & 0.187          & 0.265          & \multicolumn{1}{c|}{\textbf{0.186}}         & 0.269          & 0.213          & \multicolumn{1}{c|}{0.376}          & 0.37                                & \textbf{0.37}  & 2.11           &                \\
\model-DeepVAR & 0.035          & 0.094          & 0.193          & 0.251          & \multicolumn{1}{c|}{0.285}          & 0.242          & 0.217          & \multicolumn{1}{c|}{0.328}          & 0.44                                & 0.61           & 2.01           &                \\
\model-NoCoherent    & 0.49           & 0.117          & 0.93           & 0.258          & \multicolumn{1}{c|}{0.167}          & 0.227          & 0.193          & \multicolumn{1}{c|}{0.381}          & 0.42                                & \textbf{0.36}  & 2.18           &            \\   
\model            & \textbf{0.031} & \textbf{0.074} & \textbf{0.133} & \textbf{0.216} & \multicolumn{1}{c|}{0.252}          & \textbf{0.216} & \textbf{0.133} & \multicolumn{1}{c|}{0.338}          & \textbf{0.32}                       & 0.43           & 1.89           &                
\end{tabular}
\caption{Average CRPS scores at each level of hierarchy for \model and all variants. \model has comparable or better performance to all variants at each level of hierarchy.}
\label{tab:levels2}
\end{table*}
 

==> Text/table_var.tex <==
\begin{table*}[h]
\centering
\begin{tabular}{c|cc|cc|cc|cc|cc}
  Models/Data                 & \multicolumn{2}{c|}{Tourism-L} & \multicolumn{2}{c|}{Labour}    & \multicolumn{2}{c|}{Wiki}      & \multicolumn{2}{c|}{Flu-Symptoms} & \multicolumn{2}{c}{FB Symptoms} \\ \hline
        & CRPS           & LS            & CRPS           & LS            & CRPS           & LS            & CRPS             & LS             & CRPS           & LS             \\
\model-FineTune      & 0.16           & 0.39          & 0.031          & 0.36          & 0.216          & 0.39          & \textbf{0.240}            & \textbf{0.3}            & \textbf{1.18}           & 0.72           \\
\model-Global        & \textbf{0.13}           & 0.42          & \textbf{0.027}          & 0.31          & 0.185          & 0.34          & 0.350            & 0.47           & 2.64           & 1.39           \\
\model-DeepVAR    & \textbf{0.13}           & 0.52          & 0.029          & 0.58          & 0.201          & 0.48          & 0.361            & 0.54           & 2.13           & 0.75           \\
\model-NoCoherent & 0.18           & 0.37          & 0.043          & 0.45          & 0.227          & 0.47          & 0.248            & 0.36           & \textbf{1.17}           & 0.84   \\       
\model               & \textbf{0.12}  & \textbf{0.33} & \textbf{0.026} & \textbf{0.21} & \textbf{0.184} & \textbf{0.35} & \textbf{0.250}   & \textbf{0.28}  & 1.43  & \textbf{0.45}  
\end{tabular}
\caption{Average CRPS and IS (accros 5 runs) across all levels for \model and its variants. \model's performance is best or comparable to the best variant across all benchmarks.}
\label{tab:tab_var}
\end{table*}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

